Solution-Hashing Search Based on Layout-Graph Transformation for Unequal Circle Packing

The problem of packing unequal circles into a circular container stands as a classic and challenging optimization problem in computational geometry. This study introduces a suite of innovative and efficient methods to tackle this problem. Firstly, we present a novel layout-graph transformation method that represents configurations as graphs, together with an inexact hash method facilitating fast comparison of configurations for isomorphism or similarity. Leveraging these advancements, we propose an Iterative Solution-Hashing Search algorithm adept at circumventing redundant exploration through efficient configuration recording. Additionally, we introduce several enhancements to refine the optimization and search processes, including an adaptive adjacency maintenance method, an efficient vacancy detection technique, and a Voronoi-based locating method. Through comprehensive computational experiments across various benchmark instances, our algorithm demonstrates superior performance over existing state-of-the-art methods, showcasing remarkable applicability and versatility. Notably, our algorithm surpasses the best-known results for 56 out of 179 benchmark instances while achieving parity with the remaining instances.

==> 01Intro.tex <==
The Circle Packing Problem (CPP) %is a well-studied class of optimization problems in the field of 
 represents a fundamental challenge in computational geometry%. The objective of CPP is to find an arrangement of circles, whether congruent or of varying sizes, in a given bounded or unbounded space while ensuring that no overlapping occurs. 
,  aiming to arrange circular items optimally within a defined space while preventing overlap. 
%In most CPP studies, finding an arrangement with the maximum packing density is required
In most cases, the goal is to achieve the maximum packing density~\citep{zeng2018adaptive,stoyan2020optimized,lai2023perturbation,amore2023efficient}.
%In addition, %there are a lot of CPP variants. 
This problem encompasses various variants, each introducing additional constraints or requirements%. 
%For instance, the bin-packing variant  %aims to discover an arrangement with focuses on minimizing the number of bins required to accommodate all the circles~\citep{he2017greedy,he2021adaptive,yuan2022adaptive},   the variant involving balanced constraints or equilibrium requirements demands finding a balanced arrangement~\citep{he2013coarse,stetsyuk2016global,liu2016heuristic,wang2019stimulus,romanova2022balanced}.
, such as bin-packing~\citep{he2017greedy,he2021adaptive,yuan2022adaptive} and balanced constraints~\citep{he2013coarse,stetsyuk2016global,liu2016heuristic,wang2019stimulus,romanova2022balanced}. 
%It has been proven that CPP is an NP-hard problem~\citep{fowler1981optimal,demaine2016circle}, which indicates that finding an optimal solution is computationally challenging. Consequently, considerable efforts have been devoted to tackling various CPPs.   
Despite its computational complexity as an NP-hard problem~\citep{fowler1981optimal,demaine2016circle}, significant efforts have been dedicated to addressing CPP, 
including the Packing Unequal Circles in a Circle (PUCC) problem, which holds wide-ranging applications across industries and academia.
%One of the most classic and representative members of the CPP family is the Packing Unequal Circles in a Circle (PUCC) problem. %Wherein, the Packing Unequal Circles in a Circle (PUCC) problem is one of the classic and representative members of the CPP family.
%In this study, we address %one of the classic and representative members of the CPP family, 
%one of the most classic and representative problems, the Packing Unequal Circles in a Circle (PUCC) problem.

In this study, we address the PUCC problem, formulated as follows. 
Given $n$ circles $\{ c_1, c_2, ..., c_n \}$ with known radii $\{ r_1, r_2, ..., r_n \}$ ($r_1 \leq r_2 \leq ... \leq r_n$), PUCC consists of packing all the $n$ circles into a circular container without overlapping such that the radius of the circular container is minimized. Formally, PUCC can be formulated in the two-dimensional Cartesian coordinate system as a nonlinear programming problem as follows:
\begin{align}
    \min \quad & R \label{eq:tar} \\
    {\rm s.t.} \quad & \sqrt{{(x_{i} - x_{j})}^2 + {(y_{i} - y_{j})}^2} \geq r_{i} + r_{j}, \enskip 1 \leq i < j \leq n, \label{eq:pre1} \\ 
    \quad & \sqrt{x_{i}^{2} + y_{i}^{2}} + r_{i} \leq R, \enskip 1 \leq i \leq n, \label{eq:pre2}
\end{align}
where coordinates $(x_{i}, y_{i})$ and $(x_{j}, y_{j})$ denote the centers of circles $c_i$ and $c_{j}$, respectively, and $R$ is the radius of the circular container centered at the origin $(0, 0)$. 
%Constraints \ref{eq_pre:con1} and \ref{eq_pre:con2} ensure that all $n$ circles are contained in the circular container without any overlaps.
Constraints (\ref{eq:pre1}) and (\ref{eq:pre2}) ensure that all circles are contained in the container with no overlap. 

PUCC finds a wide range of applications in industries, such as circular cutting, container loading, cylinder packing, facility dispersion~\citep{castillo2008solving}, satellite packaging~\citep{wang2019stimulus}, etc. It is also utilized in data visualization and analysis tasks~\citep{wang2006visualization,murakami2015clonepacker,gortler2017bubble}. 
Moreover, PUCC  has attracted significant interest in academia. Al Zimmermann's Programming Contest (AZPC, see \href{http://recmath.com/contest/CirclePacking/index.php}{http://recmath.com/contest/CirclePacking/index.php}, 2006) was organized in autumn/winter of 2005,  focusing on finding the densest packing arrangements for varying numbers of circles ($n = 5, 6, ..., 50$) with integer radii ($r_{i} = i, 1 \leq i \leq n$) within a circular container.  The contest attracted 155 participants, resulting in numerous noteworthy studies and the development of 
various methods~\citep{addis2008efficiently,muller2009packing,schneider2009ultrametricity,carrabs2014tabu}.
 
In the past decade, significant efforts have continually been devoted to tackling this problem~\citep{ye2013iterated,huang2013tabu,lopez2013packing,lopez2016formulation,zeng2016iterated}, achieving impressive performances and have set many new records in terms of computational results.
Despite the extensive research history and the multitude of proposed methods and algorithms for the PUCC problem, 
finding an optimal configuration remains highly challenging due to its NP-hard nature. Moreover, obtaining high-quality configurations for moderate-scale and large-scale instances is extremely time-consuming. Therefore, the development of advanced algorithms for PUCC is crucial. Not only can these algorithms facilitate the resolution of numerous real-world applications, but they also contribute significantly to the advancement of computer science and geometry research.


In this study, we propose a new stochastic optimization algorithm, named the Iterative Solution-Hashing Search (I-SHS) algorithm, based on a classic penalty model to solve the PUCC problem. The I-SHS algorithm has a hierarchical structure consisting of multiple optimization phases. The main search ingredient is a solution-hashing search heuristic that relies on our proposed novel layout-graph transformation and solution-hashing techniques. Based on these proposed methods, our algorithm can record the explored solutions and avoid duplicate explorations during the search, enabling the algorithm to efficiently discover high-quality configurations.

Besides, we further design several methods to enhance the optimization phases of the I-SHS algorithm.
Firstly, we introduce the Adaptive Adjacency Maintenance (AAM) method, which focuses on maintaining the circle adjacency set during the layout optimization process. The AAM method incorporates two variables, namely the deferring counter and the deferring length, to calculate an adaptive maintenance feature, which would trigger the maintenance process when necessary and hence unnecessary maintenance is deferred,  reducing the computational overhead. 
Secondly, we propose an efficient vacancy detection method that utilizes continuous optimization techniques. The goal is to locate and measure vacancies in a configuration by solving a series of continuous optimization problems.
Additionally, leveraging the characteristics of two-dimensional packing problems, we introduce a Voronoi-based locating method to assist the vacancy detection method in detecting vacancies. 
By combining the latter two methods, our proposed algorithm is capable of accurately and efficiently detecting vacancies for any given configuration. 

Experiments are conducted on a range of benchmark instances with diverse radius distributions. The computational results demonstrate that our proposed algorithm significantly outperforms the state-of-the-art methods in the literature, delivering a remarkable performance in solving the PUCC problem. Specifically, our algorithm improves the best-known results for 56 out of 179 benchmark instances and matches the best-known results for the remaining instances. Furthermore, we conduct in-depth experiments to thoroughly analyze and showcase the efficiency, applicability, and generality of our proposed methods.

The main contributions and innovations of this study are summarized as follows:
\begin{itemize}
    \item We propose an efficient Iterative Solution-Hashing Search (I-SHS) algorithm with outstanding applicability and generality on diverse radius instances for solving PUCC. 
    \item We propose two novel methods, denoted as the layout-graph transformation method and the solution hash method, which tackle the difficult and challenging problem of determining whether two configurations of PUCC are isomorphic or similar. 
    \item We propose two efficient and novel methods, denoted as the vacancy detection method and Voronoi-based locating method, to locate and measure vacancies for a PUCC configuration. 
    \item We propose the Adaptive Adjacency Maintenance (AAM) method for maintaining the circle adjacent set adaptively on the continuous optimization of PUCC. 
    \item Extensive experiments on various PUCC benchmarks provide abundant and valuable computational results for future comparison. Meanwhile, our algorithm yields many new best solutions on these benchmark instances. 
\end{itemize}

The rest of this paper is organized as follows. 
In Section~\ref{sec:RW}, we provide a comprehensive review of related studies in the literature. 
Section~\ref{sec:model} presents the classic penalty model for solving PUCC that is adopted in our proposed algorithm.
In Section~\ref{sec:proalg},  we delve into details of the proposed algorithm, providing a thorough explanation of its methodology. 
The experimental results and performance comparisons of the proposed algorithm are presented in Section~\ref{sec:exp}.
%Finally, in Section~\ref{sec:conclu}, we summarize our findings and outline potential research directions for future investigations.
Finally, we summarize our findings in Section~\ref{sec:conclu}.
